You Only Search Once: Single Shot Neural Architecture Search via Direct Sparse Optimization

Recently Neural Architecture Search (NAS) has aroused great interest in both academia and industry, however it remains challenging because of its huge and non-continuous search space. Instead of applying evolutionary algorithm or reinforcement learning as previous works, this paper proposes a Direct Sparse Optimization NAS (DSO-NAS) method. In DSO-NAS, we provide a novel model pruning view to NAS problem. In specific, we start from a completely connected block, and then introduce scaling factors to scale the information flow between operations. Next, we impose sparse regularizations to prune useless connections in the architecture. Lastly, we derive an efficient and theoretically sound optimization method to solve it. Our method enjoys both advantages of differentiability and efficiency, therefore can be directly applied to large datasets like ImageNet. Particularly, On CIFAR-10 dataset, DSO-NAS achieves an average test error 2.84\%, while on the ImageNet dataset DSO-NAS achieves 25.4\% test error under 600M FLOPs with 8 GPUs in 18 hours.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/3-ProposedMethod_-_save.tex <==
\section{Proposed Method}
\label{sec:proposedmethod}
The idea of this paper follows the observation that the search space can be represented by a large directed graph, of which any architecture in the search space can be represented by a sub-graph. In other word, a neural network architecture can be obtained by pruning a subset of edges and nodes in the directed graph. Figure~\ref{DAG} illustrates an example DAG, whose nodes and edges represent local computation $\O$ and information flow respectively.

\begin{wrapfigure}{l}{7cm}
	\includegraphics[angle=270,scale=0.35]{figs/graph111.pdf}
	\caption{The whole search space can be represented by a DAG. Nodes 1 and 6 are input and output respectively, any architecture can be obtained by pruning a subset of edges and nodes in the DAG.}
	\label{DAG}
\end{wrapfigure}

The output of node $i$, $\x^i$ can be calculated by: 
\begin{align}
\label{equ:xx}x^{i}=O^i(\sum_{j<i}x^j)
\end{align}
Instead of applying controller or evolution, we address the problem in a more simple and effective way. While searching for sub-graph, we try to delete useless connection and nodes in the large DAG, leaving the ones of great importance. To achieve this goal, we apply scaling parameter on every edge in the DAG to scale the flow of information, and the input of a node is the sum of the outputs of former nodes multiplied by the scaling parameters, equation~\ref{equ:xx} can be modified to:
\begin{align}
x^{i}=O^i(\sum_{j<i}\lambda_{j}^i x^j)
\end{align}
Where $\lambda_{j}^i$ is the scaling factor applied on the connection between node $i$ and $j$. The scaling factor $\lambda$ relaxing the search space to be continues and differentiable. The sparsity constraint is applied on $\lambda$ during training to push them to zero. When $\lambda_{j}^i$ is zero, the corresponding edge can be removed safely. In the searching precess, the weights of architecture and scaling factors $\lam$ are updated alternately As weights and $\lambda$ are optimized together while training and a effective sparsity optimizer proposed by (\cite{SSS2018}) is applied.

In the following, we introduce the optimizer of our method in section~\ref{section:sss}. We then describe our search space in the form of directed acyclic graph in section~\ref{section:search space}. Finally, we introduce the searching algorithm and give a summary of SSNAS in section~\ref{section:opt and train}.

\subsection{Overview of Sparse Structure Selection} \label{section:sss}
Sparse Structure Selection was proposed by (\cite{SSS2018}) to prune network structure successfully. Instead of directly pushing the weights of network to zero, (\cite{SSS2018}) introduce a new kind of parameter $\lam$ to scale the outputs of specific structures like neurons, groups or blocks. sparsity constraint is added on $\lam$ during training to pushing $\lam$ to be sparse, if certain $\lam$ if zero, the corresponding structure can be removed as it make no contribution to the network. $\lam$ is updated by APG during training:
\begin{align}
\label{equ:z}\vz_{(t)}&=\lam'_{(t-1)}-\eta_{(t)}\nabla \MG(\lam'_{(t-1)})\\
\label{equ:v}\vv_{(t)}&=S_{\eta_{(t)}\gamma}(\z_{(t)})-\lam'_{(t-1)}+\mu_{(t-1)}\v_{(t-1)}\\
\label{equ:lam}\lam'_{(t)}&=S_{\eta_{(t)}\gamma}(\vz_{(t)})+\mu_{(t)}\vv_{(t)}
\end{align}
In practice, (\cite{SSS2018}) follow a stochastic approach with mini-batches and $\mu$ is fixed to a constant value. Weights and $\lam$ are updated in each iteration. The depth and width can be adaptively adjusted by adjusting the sparse constrain on $\lam$. (\cite{SSS2018}) shows very promising acceleration performances on the CIFAR datasets and the large scale ILSVRC2012 image classification datasets. However, Sparse Structure Selection can only modify the structure like channels, blocks of exiting architecture, with no ability to discover novel architecture within a rich search space. Instead of applying scaling factors on the outputs of structure, we apply $\lam$ to scale the connection in the cell, getting rid of the limitation of relaying on exiting architecture. Through scaling and pruning, SSNAS can obtain a new architecture with state-of-the-art performance.

\subsection{Search Space} \label{section:search space}
As well as searching for building cell just as (\cite{pham2018efficient}) do, SSNAS can alos be applied to search for whole network, still keeping a competitive searching time.  We assume that the architecture is hierarchical and cell is stacked for a certain number of time.

A cell is a directed acyclic graph consisting of an ordered sequence of $M$ layers, every layer consists of the $N$ operations. The structure of cell is illustrated in Figure~\ref{method}. Every operation is connected to the input of cell and operations in the formal layers with a scaling factor $\lambda$, the input of operation is the sum of all outputs of previous nodes multiplied by the scaling factors. The output of the $j$ th operation in $i$ th layer $x_{i,j}$ is computed based on all of its predecessors:
\begin{align}
\label{equ:x}\tX_{(i,j)}=O_{(i,j)}(\sum_{m<i,n\in(1,N)}\lam_{(m,n)}^{(i,j)}\tX_{(m,n)} + \lam^{(i,j)}\tI)
\end{align}
\begin{figure*}[htbp]
	\centering
	\subfigure[]{
		\begin{minipage}[t]{0.3\linewidth}
			\centering
			\includegraphics[scale=0.25]{figs/graph3-1.pdf}
		\end{minipage}
	}
	\subfigure[]{
		\begin{minipage}[t]{0.3\linewidth}
			\centering
			\includegraphics[scale=0.25]{figs/graph3-2.pdf}
		\end{minipage}
	}
	\subfigure[]{
		\begin{minipage}[t]{0.3\linewidth}
			\centering
			\includegraphics[scale=0.25]{figs/graph3-3.pdf}
		\end{minipage}
	}
	\centering
	\caption{An searching process of two-layer-block, which has two layers with two operations:(a)Edges are applied with a scaling factor $\lam$, which is trained with Sparse Structure Selection~\cite{SSS2018}. (b)Any edge whose $\lam$ is zero can be removed safely as no contribution is made to the network. (c)Generating new architecture by pruning useless edges and operations.}
	\label{method}
\end{figure*}
Where $O_{m,n}$ is the local computation of the $n$ th operation in $m$ th layer and $\tI$ is the input of block. The connections between operations and output of cell are also learn-able with scaling factors $\lam$ applied on the corresponding connections. The output of the block $\tO$ is obtained by applying a reduction operation(e.g.concatenation) $C$ to all the nodes that have  contribution to the output:
\begin{align}
\label{equ:O}\tO=C(\sum_{m,n}\lam_{(m,n)}\tX_{(m,n)})+id
\end{align}
Identity mapping is applied between the input and output in case all operations are pruned. We include following four kinds of operations in convolution cell: separable convolution with kernel 3$\times$3 and 5$\times$5, average pooling and max pooling with kernel 3$\times$3. 
As for reduction block,we simply use normal convolutions with kernel size 1$\times$1 and 3$\times$3, and apply them with a stride of 2 to reduction feature map and double the number of filters.
The task of searching block therefore reduces to learning $\lam$ on every edges. Thus the architecture searching problem has been reformulated as a sparse problem:
\begin{align}
\min_{\mW,\lam}\frac{1}{N}\sum_{i=1}^{N}L(\tY_i,Net(\tX_i,\mW,\lam))+R_s(\lam)
\end{align}
Where $R_s(.)$ is a sparsity regularization for $\lam$, $\tX_i$ and $\tY_i$ are input data and label respectively, $\mW$ represents the weights of the network.

\subsection{Optimization and Training} \label{section:opt and train}
In SSNAS, there are two kinds of learn-able parameters: the weights of the network $\mW$ and the structure parameters $\lam$. We updata $\mW$ with NAG and APGNAG proposed by \cite{SSS2018} for $\lam$. However, in \cite{SSS2018}, the weight and $\lam$ are updated together in same training set, which may cause overfitting in small datasets like CIFAR-10, leading to the poor performance of network. To solve this problem, we divide training set into two parts, training set and validation set, the weights of network $\mW$ are updated in the training set and structure parameters $\lam$ are updated in the validation set. The scalers in batch normalizations are fixed during searching process to prevent their effect to $\lam$. To keep the balance among different cells and prevent necessary operation from being pruned. We adjust the intensity of regularity, $\gamma$ adaptively according to the flops in the block. When optimizing $\lam$ using APGNAG, $\gamma$ in ~\ref{equ:v}~\ref{equ:lam} is calculating by:
\begin{align}
\label{equ:gamma}\gamma_{iter}=\frac{\b{FLOPS}_{iter}}{\b{FLOPS}_{block}}\gamma
\end{align}
where $\b{FLOPS}_{block}$ represents the flops of the block keeping all operation and $\b{FLOPS}_{iter}$, which can be calculating based on $\lam$ represents the flops in the process of searching. Using this strategy, we can prevent cells from making no contribution to the network by prevent all operation from being pruned.
\begin{algorithm}
	\caption{SS-NAS}
	\label{alg:A}
	\begin{algorithmic}
		\STATE update $\vw$ by optimizing $L_{train}(\mW)$ for several epochs
		\REPEAT
		\STATE update $\vw$ by optimizing $L_{train}(\mW,\lam)$
		\STATE update $\lam$ by optimizing $L_{val}(\mW,\lam)$
		\UNTIL{converged} 
	\end{algorithmic}
\end{algorithm}
We denote the loss on two datasets as $L_{train}(\mW,\lam)$ and $L_{val}(\mW,\lam)$ respectively, and the task of searching architecture is to find the $w^*$ that minimizing the $L_{train}(\mW^*,\lam)$ and $\lam^*$ that minimizing the $L_{val}(\mW,\lam^*)$. We also find it important to update $\mW$ for several epochs in training set with $\lam$ fixed to obtain good architecture as the searching process is highly depend on the performance of architecture.

==> sections/4-Experiments_-_save.tex <==
\section{Experiments}
\label{sec:experiments}
The searching process can be divided into following three stages:(1) A large network consisting of all operations and connections is trained for several epoch to specify the importance of connections and operations . (2) In the searching process, the structure parameter $\lam$ and weights are trained together with sparse regulation applied on the $\lam$. (3) The searched architecture is trained from scratch and evaluated on test data. In the first two stages, the scalers in batch normalizations are fixed during searching process to prevent their effect to $\lam$. We apply SSNAS in two search spaces: 1.the micro search space where $\lambda$ is shared among cells. 2. the macro search space over whole network and $\lambda$ in different cells are updated identity. In the searching process, we find the pruned connections have little chance to reconnect as the relating weights of operations are not updated, so the pruned connections and operations are deleted every five epoch to accelerate the searching process. As for architecture evolution \footnote{where do you describe the three stage training? It is hard to understand the meaning of evolution.}, we adjust the number of filter to satisfy the computation budget and train the architecture from scratch. We test our algorithm on two famous dataset, the CIFAR-10 dataset and the Imagenet dataset. On the CIFAR-10 dataset, we search architecture on the macro search space and micro search space, we run every experiment for five times and report the mean $x$ and standard deviation $y$ as $x\pm y$. As for ImageNet dataset, we evaluate the architecture searched on the CIFAR-10 dataset, proving the transform ability of the architecture and try to directly search on the ImageNet dataset directly, also achieving impressive results.

\subsection{CIFAR}
The CIFAR-10 dataset consists of 50000 training images and 10000 testing images. We divide the training data into two parts: 25000 for training and 25000 for validation. Standard data pre-processing and augmentation techniques are used including subtracting the mean and dividing the standard deviation of images, randomly flipping horizontally, padding images to 40 $\times$ 40 and randomly cropping to 32 $\times$ 32. Firstly, we train the whole model for 120 epochs with structure parameters fixed, getting a good initialize of weights, then search network batch size 128 in two GPUs until converge. NAG is applied to optimize weight $W$ with initial learning rate $lr = 0.1$, momentum 0.9, weight decay $1\times10^{-4}$. APGNAG proposed by \cite{SSS2018} is applied to optimize $\lambda$ with same initial learning rate $lr = 0.1$. In the whole searching process, test data is never used. Adoptive flops~\ref{section:opt and train} is applied in the searching process. It takes 0.5 days for two GPUs to finiash the searching process.

\begin{wrapfigure}{l}{7cm}
	\includegraphics[scale=0.30,angle=270]{figs/graph-arch.pdf}
	\caption{Convolution cell searched on CIFAR-10}
	\label{cifar_architecture}
\end{wrapfigure}

As for architecture evaluation, the searched model is trained for 640 epochs using cosine learning scheduler with batch size 128. Following existing evaluation  method~\cite{pham2018efficient,liu2018darts}, additional enhancements including dropout with probability 0.6, cutout~\cite{cutout2017} with size 16, drop path with probability 0.5, auxiliary towers located at 2/3 of total length of total network with weight 0.4 are added.
The results of CIFAR-10 are shown in table~\ref{res_cifar10} and the searched architecture of cell is shown in figure~\ref{cifar_architecture}.

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{table}[htb]
	\caption{Comparison with state-of-the-art image classifiers on CIFAR-10.}
	\begin{center}
		\begin{tabular}{l c c c c c}
			\hline
			Architecture & Test Error & Params(M) & \tabincell{c}{Search Cost\\(GPU days)} & \tabincell{c}{Search \\Method}\\
			\hline
			DenseNet & 3.46 & 25.6 & - & manual\\
			\hline
			NASNet-A+cutout \cite{zoph2017learning} & 2.65 & 3.3 & 1800 & RL\\
			AmoebaNet-A \cite{real2018regularized} & 3.34 & 3.2 & 3150 & evolution\\
			AmoebaNet-B+cutout \cite{real2018regularized} & 2.55 & 2.8 & 3150 & evolution \\
			PNAS \cite{liu2017progressive} & 3.41 & 3.2 & 150 & SMBO\\
			ENAS+cutout \cite{pham2018efficient} & 2.89 & 4.6 & 0.5 & RL \\
			DARTS+cutout \cite{liu2018darts} & 2.83 & 3.4 & 4 & gradient-based \\
			\hline
			SSNAS-micro+cutout & 2.84 $\pm$ 0.07& 3.0 & 1 & gradient-based \\
			SSNAS-macro+cutout & 2.95 $\pm$ 0.12 & 3.0 & 1 & gradient-based \\
			random-micro + cutout & 3.58 $\pm$ 0.21 & 3.4 $\pm$ 0.1 & - & - \\
			random-macro + cutout & 3.52 $\pm$ 0.19 & 3.5 $\pm$ 0.1 & - & - \\
			\hline
		\end{tabular}
	\end{center}
	\label{res_cifar10}
\end{table}
It is obvious that SSNAS achieve comparable results with stat of the art while using much less computation resource. When compared with ENAS~\cite{pham2018efficient}, and DARRTS~\cite{liu2018darts}, SSNAS outperforms them with less parameters. Finally, it is interesting to note that searching in micro search space is slower than searching in macro search space which is due to the fact that when searching in macro search space, the operations and connections are easier to be pruned, accelerating searching process.

\subsubsection{The Effective of Flops-Aware Technique}
The flops-aware technique also play a important role in the searching process by preventing some cells from being pruned totally and balancing the distribution of FLOPS shown in figure~\ref{flops-distribution}~\ref{param-distribution}. In the searching process, the regulation intensity is changed adoptively according to equation~\ref{equ:gamma_flops}. It is obvious to see that the operation in the third stage of network are more inclined to be pruned while searching on small dataset like CIFAR-10, causing the imbalance distribution of FLOPS. With flops-aware technique, more operations in the third stage are kept, smoothing the curve of distribution of FLOPS and parameters. Figure~\ref{flop-vs-acc}~\ref{param-vs-acc} also show the promise performance enhance of flops-aware technique under same computation budget.
\begin{figure*}[htbp] 
	\centering
	\subfigure[]{
		\begin{minipage}[t]{0.42\linewidth}
			\centering
			\includegraphics[scale=0.4]{figs/figure-flops.pdf}
		\end{minipage}
		\label{flops-distribution}
	}
	\subfigure[]{
		\begin{minipage}[t]{0.42\linewidth}
			\centering
			\includegraphics[scale=0.4]{figs/figure-param.pdf}
		\end{minipage}
		\label{param-distribution}
	}
	\subfigure[]{
		\begin{minipage}[t]{0.42\linewidth}
			\centering
			\includegraphics[scale=0.4]{figs/graph_adflops.pdf}
		\end{minipage}
		\label{flop-vs-acc}
	}
	\subfigure[]{
		\begin{minipage}[t]{0.42\linewidth}
			\centering
			\includegraphics[scale=0.4]{figs/graph_adparam.pdf}
		\end{minipage}
		\label{param-vs-acc}
	}
	\caption{(a)(b) Comparison of FLOPS and parameters distribution. By using flops-aware technique, the curve of distribution of flops is more smoother. (c)(d)Error rates vs number of parameters and FLOPS, we can see guarantee performance enhancement of flops-aware technique under certain computation budget.}
	\centering
	\label{distribution}
\end{figure*}

\subsubsection{The Effective of Adoptive MAC Technique}

\begin{wrapfigure}{l}{7cm}
	\includegraphics[scale=0.40]{figs/graph_admac.pdf}
	\caption{Error Vs number of MAC with adoptive MAC technique}
	\label{mac-vs-acc}
\end{wrapfigure}

SSNAS can also search architecture based on certain computational target, take MAC for example. We also try to optimize MAC in the searching process by penaltying the connections related to high-MAC-operations with larger regulation intensity, forcing architecture to select MAC-saving operation. The number of MAC of every operation is calculated and normalized by the maximum number of MAC and regulation intensity is calculated according to equation~\ref{equ:gamma_mac}. The result is shown in figure~\ref{mac-vs-acc}. It is obvious to see that SSNAS can generate architecture with higher accuracy under certain MAC budget, proving the effectiveness of adoptive MAC technique. The similar method can be applied to optimize many other computation budget like number of parameters, FLOPS, which can leave for further study.

\subsubsection{Other Factors For Searching Architecture}
The searching process may be affected by many other hyper-parameters or settings, we do experiment on different setting of architecture searching for further research work. The result is shown in table~\ref{com_cifar10}.

\begin{table}[htb]
	\caption{Comparison of different setting while search on the CIFAR-10 dataset in the macro search space.}
	\begin{center}
		\begin{tabular}{c c c c c}
			\hline
			split training & Ratio of T\&V &Initialize & Params(M) & Test Error  \\
			\hline
			Yes & 4:1  & pretrain & 2.9 & 3.05 $\pm$ 0.09\\
			Yes & 1:1 & random & 2.9 & 3.26 $\pm$ 0.08\\
			No & -  & pretrain & 3.0 & 3.20 $\pm$ 0.1\\
			Yes & 1:1 & pretrain & 3.0 & 3.02 $\pm$ 0.09\\
			\hline
		\end{tabular}
	\end{center}
	\label{com_cifar10}
\end{table}

where Ratio of T\&V means the ratio of images number in training set and validation set, as for ratio of training and validation set $x:y$, we update weight for $x$ times and update $\lam$ for $y$ times for every $x+y$ iterations. Initialize means whether to search architecture based on pretrain model or from scratch while split training means whether to split the whole training set into training set and validation set. The pretrain model is only trained on the training set. It is notable that the utilize of validation set plays an important role in the search process as it help prevent architecture from overfitting training data and improve the performance by 0.2\% while the ratio of training set and validation set has little influence. Besides, the good initialize of weight if also of great importance as random initialize of weight may lead to a 0.3\% drop on accuracy under same parameter budget.

\begin{comment}
%Just like the experiment in CIFAR-10, we divide the dataset into two parts, 25000 for training and 25000 for validation. Other settings of network is the same as the settings in CIFAR-10. Firstly, we train the whole model for 120 epochs with $\lambda$ fixed, and search network using SSNAS, with batch size 128 in two GPUs.

%As for architecture evaluation, the model is trained for 640 epochs, with batch size 128, initial learning rate 0.05, additional enhancements including dropout with probability 0.8, cutout with size 8, drop path with probability 0.7.

\begin{table}[htb]
	\caption{Comparison with state-of-the-art image classifiers on CIFAR-100}
	\begin{center}
		\begin{tabular}{c c c c c c}
			\hline
			Architecture & Test Error & Params(M) & \tabincell{c}{Search Cost\\(GPU days)} & \tabincell{c}{Search \\Method}\\
			\hline
			DenseNet+cutout \cite{baker2016cutout} & 15.20 & 25.6 & - & manual\\
			\hline
			MetaQNN(top model) \cite{baker2016designing} & 27.14 & - & 80 & LR\\
			Block-QNN-A,N=4 \cite{zhong2018practical} & 18.64 & - & 96 & LR\\
			Block-QNN-B,N=4 \cite{zhong2018practical} & 18.72 & - & 96 & LR\\
			\hline
			SSNAS & 18.43 & 3.0 & 2 & gradient-based\\
			\hline
		\end{tabular}
	\end{center}
\end{table}
\end{comment}

\subsection{ILSVRC 2012}
As for architecture searching on the ImageNet dataset, we consider the mobile setting of ImageNet where the input image size if 224$\times$224. We also divide the training data into two parts: four fifths for training and one fifth for validation. We firstly pretrain the whole network with 27 cells for 30 epochs with learing rate 0.1, weight decay 4e-5, and search network with batch size 256 in eight GPUs. In the searching process, the pruned connection and operations are deleted to accelerate searching process every epoch just like the searching process on the CIFAR dataset.

As for architecture evaluation, the searched model is trained using NAG for 240 epochs in eight GPUs, with batch size 1024, weight decay $4\times10^{-5}$ and initial learning rate 0.1 (gradually raise to 0.5 in five epochs and drop linearly to 0 in the rest epochs). We restrict the number of multi-adds to around 600M. Additional enhance including smoothing label and auxiliary towers located at the second to last stages of network. We evaluate the architecture of cell searched on the CIFAR-10 dataset and the architecture searched directly on the ImageNet, the results for ImageNet are shown in table~\ref{imagenet}, where results marked with * were obtained by searching on the CIFAR-10 dataset.

\begin{table}[ht]
	\caption{Comparison with state-of-the-art image classifiers on ImageNet}
	\begin{center}
		\begin{tabular}[h]{c c c c c}
			\hline
			Architecture & Top-1/5 & Params(M) & FLOPS(M) &\tabincell{c}{Search Cost\\(GPU days)} \\
			\hline
			Inception-v1 \cite{szegedy2015going} & 30.2/10.1 & 6.6 & 1448 & - \\
			MobileNet \cite{howard2017mobilenets} & 29.4/10.5 & 4.2 & 569 & - \\
			ShuffleNet-v1 2x \cite{shufflenet} & 26.3/10.2 & ~5 & 524 & - \\
			ShuffleNet-v2 2x \cite{shufflenetv2} & 25.1/- & ~5 & 591 & - \\
			NASNet-A* \cite{zoph2017learning} & 26.0/8.4 & 5.3 & 564 & 1800 \\
			NASNet-B* \cite{zoph2017learning} & 27.2/8.7 & 5.3 & 488 & 1800 \\
			NASNet-C* \cite{zoph2017learning} & 27.5/9.0 & 4.9 & 558 & 1800\\
			AmoebaNet-A* \cite{real2018regularized} & 25.5/8.0 & 5.1 & 555 & 3150\\
			AmoebaNet-B* \cite{real2018regularized} & 26.0/8.5 & 5.3 & 555 & 3150 \\
			AmoebaNet-C* \cite{real2018regularized} & 24.3/7.6 & 6.4 & 570 & 3150 \\
			PNAS* \cite{liu2017progressive} & 25.8/8.1 & 5.1 & 588 & 150\\
			OSNAS \cite{OSNAS2018} & 25.8/- & 5.1 & - & - \\
			DARTS* \cite{liu2018darts} & 26.9/9.0 & 4.9 & 595 & 4\\
			\hline
			SSNAS* & 26.2/8.6 & 4.7 & 571 & 1 \\
			SSNAS-micro  & 26.1/8.4 & 4.6 & 608 & 4\\
			SSNAS-macro  & 25.7/8.4 & 4.9 & 598 & 4\\
			%SSNAS-micro & 25.9/8.3 & 4.9 & 588 & 3 & gradient-based\\
			%SSNAS-macro & 25.9/8.3 & 4.9 & 588 & 3 & gradient-based\\
			\hline
		\end{tabular}
	\end{center}
	\label{imagenet}
\end{table}
It is notable that SSNAS achieves competitive performance with the state-of-the-art architecture. The architecture searched on the CIFAR-10 dataset also achieve good performance, proving the generalization capability of architecture, besides, we find searching in macro search space yield better result, on the contrary to the experiments on the CIFAR-10 dataset, indicating searching in larger search space require more data. 

==> sections/5-Discussions.tex <==
\section{Discussions}
\label{sec:discussions}

 Then the loss of FitNet can be defined as:
\begin{equation}\label{equ:FN}
\mathcal{L}_{FN}(\textbf{W}_S)=\mathcal{H}(\bm{y}_{true},\bm{p}_S^1)+
\frac{\lambda}{2}||V(\bm{F}_T)-V(R(\bm{F}_S;\textbf{W}_R))||^2,
\end{equation}
where $R(\bm{F}_S;\textbf{W}_R)$ is a convolutional regressor which converts $\bm{F}_S$ from $\mathbb{R}^{C_S \times H \times W}$ to $\mathbb{R}^{C_T \times H \times W}$ if $C_T \neq C_S$, else it is an identity mapping, and $V(\cdot)$ is an vectorized operation. The loss of AT can be formulated by following:
\begin{equation}\label{equ:AT}
\mathcal{L}_{AT}(\textbf{W}_S)=\mathcal{H}(\bm{y}_{true},\bm{p}_S^1)+
\frac{\lambda}{2}||V(A(\bm{F}_T))-V(A(\bm{F}_S))||^2,
\end{equation}
where $A(\bm{F})$ is an attention mapping which has several definitions \cite{Zagoruyko2017AT}, such as sum of absolute values defined by:
\begin{equation}\label{equ:sumabs}
A_{abssum}(\bm{F})=\sum_{k=1}^{C}{|\bm{F}^k|}.
\end{equation}
Substituting Eq. \ref{equ:sumabs} into Eq. \ref{equ:AT}, we can get:
\begin{equation}\label{equ:sumabsAT}
\mathcal{L}_{AT_{S}}(\textbf{W}_S)=\mathcal{H}(\bm{y}_{true},\bm{p}_S^1)+
\frac{\lambda}{2}||\sum_{i=1}^{C_T}{|\bm{f}_T^i|}-\sum_{j=1}^{C_S}{|\bm{f}_S^j|}||^2.
\end{equation}


